Deep learning for spatio-temporal forecasting -- application to solar energy

This thesis tackles the subject of spatio-temporal forecasting with deep learning. The motivating application at Electricity de France (EDF) is short-term solar energy forecasting with fisheye images. We explore two main research directions for improving deep forecasting methods by injecting external physical knowledge. The first direction concerns the role of the training loss function. We show that differentiable shape and temporal criteria can be leveraged to improve the performances of existing models. We address both the deterministic context with the proposed DILATE loss function and the probabilistic context with the STRIPE model. Our second direction is to augment incomplete physical models with deep data-driven networks for accurate forecasting. For video prediction, we introduce the PhyDNet model that disentangles physical dynamics from residual information necessary for prediction, such as texture or details. We further propose a learning framework (APHYNITY) that ensures a principled and unique linear decomposition between physical and data-driven components under mild assumptions, leading to better forecasting performances and parameter identification.

==> dedicace.tex <==
\thispagestyle{empty}

\begin{flushright}
 Insérer éventuellement une dédicace ... 


\end{flushright}

\noindent 

==> glossaire.tex <==
%----- Acronymes -----%

\newglossaryentry{usbl}{
     type=\acronymtype,
     name={USBL},
     description={système de positionnement acoustique par ligne de base ultra courte ou \emph{Ultra Short Base Line acoustic positioning system}},
     first={USBL (système de positionnement acoustique par ligne de base ultra courte ou \emph{Ultra Short Base Line acoustic positioning system})},
     }

\newglossaryentry{slam}{
     type=\acronymtype,
     name={SLAM},
     description={Localisation et cartographie simultanées ou \emph{Simultaneous Location And Mapping}},
     first={SLAM (Localisation et cartographie simultanées ou \emph{Simultaneous Location And Mapping})},
     }
     
\newglossaryentry{ascii}{
     type=\acronymtype,
     name={ASCII},
     description={Code américain normalisé pour l'échange d'information ou \emph{American Standard Code for Information Interchange}},
     first={ASCII (Code américain normalisé pour l'échange d'information ou \emph{American Standard Code for Information Interchange})},
     }
          
     
\newglossaryentry{lbl}{
     type=\acronymtype,
     name={LBL},
     description={système de positionnement acoustique par longue ligne de base ou \emph{Long BaseLine acoustic positioning system}},
     first={LBL (système de positionnement acoustique par longue ligne de base ou \emph{Long BaseLine acoustic positioning system})},
     }
     
\newglossaryentry{auv}{
     type=\acronymtype,
     name={AUV},
     description={Véhicule sous-marin autonome ou \emph{Autonomous Underwater Vehicle}},
     first={AUV (Véhicule sous-marin autonome ou \emph{Autonomous Underwater Vehicle})},     
     }
     
\newglossaryentry{uuv}{
     type=\acronymtype,
     name={UUV},
     description={Véhicule sous-marin non-habité ou \emph{Unmanned Underwater Vehicle}},
     first={UUV (Véhicule sous-marin non-habité ou \emph{Unmanned Underwater Vehicle})},     
     }
     
\newglossaryentry{rov}{
     type=\acronymtype,
     name={ROV},
     description={Véhicule téléguidé ou \emph{Remotely Operated Vehicle}},
     first={ROV (Véhicule téléguidé ou \emph{Remotely Operated Vehicle})},     
     }
     
\newglossaryentry{hrov}{
     type=\acronymtype,
     name={HROV},
     description={Véhicule téléguidé hybride ou \emph{Hybrid Remotely Operated Vehicle}},
     first={HROV (Véhicule téléguidé hybride ou \emph{Hybrid Remotely Operated Vehicle})},     
     }
     
\newglossaryentry{gravimob}{
    type=\acronymtype,
    name={GraviMob},
    description={Système de Gravimétrie Mobile ou \emph{Mobile Gravimetry System}},
    first={GraviMob (Système de Gravimétrie Mobile ou \emph{Mobile Gravimetry System})},
    }
    
\newglossaryentry{limog}{
    type=\acronymtype,
    name={LiMo-g},
    description={Système Léger de Gravimétrie Mobile ou \emph{Light Moving Gravimetry System}},
    first={LiMo-g (Système Léger de Gravimétrie Mobile ou \emph{Light Moving Gravimetry System})},
    }
    
\newglossaryentry{ldo}{
    type=\acronymtype,
    name={LDO},
    description={Laboratoire de Domaines Océaniques},
    first={LDO (Laboratoire de Domaines Océaniques)},
    }
    
\newglossaryentry{ifremer}{
    type=\acronymtype,
    name={IFREMER},
    description={Institut Français de Recherche pour l'Exploitation de la Mer},
    first={Institut Français de Recherche pour l'Exploitation de la Mer (IFREMER)},
    }
    
\newglossaryentry{ipgp}{
    type=\acronymtype,
    name={IPGP},
    description={Institut de Physique du Globe de Paris},
    first={Institut de Physique du Globe de Paris (IPGP)},
    }

\newglossaryentry{onera}{
    type=\acronymtype,
    name={ONERA},
    description={Office National d'Études et de Recherches Aérospatiales},
    first={Office National d'Études et de Recherches Aérospatiales (ONERA)},
    }

\newglossaryentry{shom}{
    type=\acronymtype,
    name={SHOM},
    description={Service Hydrographique et Océanographique de la Marine},
    first={Service Hydrographique et Océanographique de la Marine (SHOM)},
    }    
    
\newglossaryentry{grs80}{
    type=\acronymtype,
    name={GRS80},
    description={Système de Référence Géodésique 1980 ou \emph{Geodetic Reference System 1980}},
    }
    
\newglossaryentry{svd}{
    type=\acronymtype,
    name={SVD},
    description={Décomposition en Valeurs Singulières ou \emph{Singular Value Decomposition}},
    first={décomposition en valeurs singulières ou \emph{Singular Value Decomposition} (SVD)},
    }   

\newglossaryentry{esgt}{
    type=\acronymtype,
    name={ESGT},
    description={École Supérieure des Géomètres et Topographes},
    first={École Supérieure des Géomètres et Topographes~(ESGT)},
    } 
    
\newglossaryentry{egm08}{
    type=\acronymtype,
    name={EGM2008},
    description={\emph{Earth Gravitational Model 2008}},
    first={EGM2008 (\emph{Earth Gravitational Model 2008})},
    } 

\newglossaryentry{odp}{
    type=\acronymtype,
    name={OP},
    description={Observatoire de Paris},
    first={Observatoire de Paris (OP)},
    } 

\newglossaryentry{ign}{
    type=\acronymtype,
    name={IGN},
    description={Institut National de l'information Géographique et forestière},
    first={Institut National de l'information Géographique et forestière (IGN)},
    } 

\newglossaryentry{lareg}{
    type=\acronymtype,
    name={LAREG},
    description={Laboratoire de Recherche en Géodésie},
    first={Laboratoire de Recherche en Géodésie (LAREG)},
    } 
    
\newglossaryentry{gps}{
    type=\acronymtype,
    name={GPS},
    description={Système Global de Positionnement ou \emph{Global Positioning System}},
    first={GPS (Système Global de Positionnement ou \emph{Global Positioning System})},
    } 
    
\newglossaryentry{mems}{
    type=\acronymtype,
    name={MEMS},
    description={Microsystème électromécanique ou \emph{Microelectromechanical systems}},
    first={MEMS (Microsystème électromécanique ou \emph{Microelectromechanical systems})},
    } 
%----- Définition -----%

\newglossaryentry{i-frame}{
	name={\emph{i-frame}},
	description={le \emph{i-frame} (ou \emph{inertial-frame}) désigne le repère accompagnant la Terre dans son mouvement de translation elliptique autour du Soleil},
	}    

\newglossaryentry{e-frame}{
	name={\emph{e-frame}},
	description={le \emph{e-frame} (ou \emph{earth-frame}) désigne le repère accompagnant la Terre dans son mouvement de rotation sur elle-même},
	} 

\newglossaryentry{n-frame}{
	name={\emph{n-frame}},
	description={le \emph{n-frame} (ou \emph{navigation-frame}) désigne le repère géographique local},
	first={\emph{n-frame}},
	}    
    
\newglossaryentry{b-frame}{
	name={\emph{b-frame}},
	description={le \emph{b-frame} (ou \emph{body-frame}) désigne le repère attaché au véhicule porteur},
	first={\emph{b-frame}},
	}

\newglossaryentry{alpha-frame}{
	name={$s_{\alpha}$\emph{-frame}},
	description={le $s_{\alpha}$\emph{-frame} (resp. $s_{\beta}$\emph{-frame}) (ou \emph{system-frame}) est le repère attaché à la triade accélérométrique $\alpha$ (resp. $\beta$)},
	first={$s_{\alpha}$\emph{-frame}},
	}
	
\newglossaryentry{beta-frame}{
	name={$s_{\beta}$\emph{-frame}},
	description={le $s_{\alpha}$\emph{-frame} (resp. $s_{\beta}$\emph{-frame}) (ou \emph{system-frame}) est le repère attaché à la triade accélérométrique $\alpha$ (resp. $\beta$)},
	first={$s_{\beta}$\emph{-frame}},
	}

%----- Symboles -----%     
     
\newglossaryentry{delta}{
     type=notation,
     name={\ensuremath{\delta}},
    description={Angle de cap},
    sort={delta}
     }





==> page_garde_president.tex <==
\thispagestyle{empty}

\newgeometry{
        showframe,
		top=20mm,
		bottom=20mm,
		inner=20mm,
		outer=20mm,
		includehead,
		ignorefoot,
		nomarginpar,
		headsep=10mm,
		footskip=10mm,
	}


\setmarginsrb{5mm}{5mm}{18mm}{5mm}{0mm}{0mm}{0mm}{0mm}


\resizebox{\textwidth}{!}{

\begin{tabular}{p{11cm}p{5cm}}
		\begin{minipage}{11cm}
                \vspace{0.5cm}
			\begin{center}
				\textbf{\LARGE{}}
			\end{center}
                \vspace{1.cm}
		\end{minipage}
	&
		\begin{minipage}{5cm}
		\vspace{1cm}
		\begin{center}
			\includegraphics[width=0.9\textwidth]{images/Cnam.jpg}
			\end{center}
			\vspace{0.25cm}
		\end{minipage}
\end{tabular}
}

%\renewcommand\aromesurei{.22cm}

%\begin{center}
\vspace{1cm}
\makebox[\textwidth][c]{\centering{\LARGE{\textbf{\'ECOLE DOCTORALE Nom de l'école}}}}\\
\vspace{0.5cm}
\hspace{0.5cm}\makebox[\textwidth][c]{\centering{\LARGE{\textbf{Nom du laboratoire de recherche}}}}\\
\vspace{0.5cm}
\makebox[\textwidth][c]{{\LARGE{\textbf{TH\`ESE DE DOCTORAT}}}}\\
\vspace{1cm}
\makebox[\textwidth][c]{\centering{\large{\textit{présentée par} : }} {\Large{\textbf{Prénom NOM}}}}\\
\vspace{.4cm}
\makebox[\textwidth][c]{\centering{\large{\textit{soutenue le} : }} {\Large{\textbf{XX mois en lettres 20XX}}}}\\
\vspace{.4cm}
\makebox[\textwidth][c]{\centering{\large{\textit{pour obtenir le grade de} : }} {\large{\textbf{Docteur du Conservatoire National des Arts et Métiers}}}}\\
\vspace{.4cm}
\makebox[\textwidth][c]{\centering{\large{\textit{Discipline} :}} {\large{\textbf{Discipline CNU a compléter}}}}
\makebox[\textwidth][c]{\centering{\large{\textit{Spécialité} :}} {\large{\textbf{Spécialité}}}}
			\vspace{1cm}

%\end{center}

\resizebox{\textwidth}{!}{
\fbox{
\begin{tabular}{>{\centering\arraybackslash}p{16.5cm}}
\begin{minipage}{16.5cm}
\centering
\vspace{0.2cm}
{\LARGE{\textbf{{Titre de la thèse}}}}\\
%{\LARGE{\textbf{{}}}}
\vspace{0.2cm}
\end{minipage}	
\end{tabular}
}}~\\

\vspace{.22cm}

\vfill


%\renewcommand\aromesurei{.2cm}
\hspace{0.7cm}\textbf{\textsc{\large TH\`{E}SE dirig\'{e}e par }} \\ \vspace{.2cm}
\hspace{0.7cm}\begin{tabular}{p{0.5cm} p{7cm} p{10cm}}
	& Civilité \textsc{Nom} Prénom &  \textit{Titre, établissement}\\
\end{tabular}

\vspace{.4cm}

\hspace{0.7cm}\textbf{et co-encadré par}  \\\vspace{.2cm}
\hspace{0.7cm}\begin{tabular}{p{0.5cm} p{7.cm} p{10cm}}
 	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
\end{tabular}

\vspace{.4cm}

\hspace{0.7cm}\textbf{\textsc{RAPPORTEURS }}  \\\vspace{.2cm}
\hspace{0.7cm}\begin{tabular}{p{0.5cm} p{7.cm} p{10cm}}
 	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
\end{tabular}

\vspace{.4cm}


\hspace{0.7cm}\textbf{\textsc{PR\'{E}SIDENT DU JURY }}  \\ \vspace{.2cm}
\hspace{0.7cm}\begin{tabular}{p{0.5cm} p{7.cm} p{10cm}}
	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
\end{tabular}

\vspace{.4cm}

\hspace{0.7cm}\textbf{\textsc{EXAMINATEURS  } } \\ \vspace{.2cm}
\hspace{0.7cm}\begin{tabular}{p{0.5cm} p{7.cm} p{10cm}}
	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
\end{tabular}

\vspace{.4cm}

\hspace{0.7cm}\textbf{\textsc{MEMBRES INVIT\'{E}S } } \\ \vspace{.2cm}
\hspace{0.7cm}\begin{tabular}{p{0.5cm} p{7.cm} p{10cm}}
	& Civilité \textsc{Nom} Prénom   &  \textit{Titre, établissement}  \\
\end{tabular}




%
%\vspace{.5cm}
%
%
%\textbf{\textsc{MEMBRE INVIT\'{E}}}  \\ \vspace{.2cm}\begin{tabular}{p{0.5cm} p{5.cm} p{12cm}}
%	&M. \textsc{Pouliguen} Philippe &  \textit{Responsable du Domaine Scientifique "Ondes Acoustiques et Radioélectriques", DGA}
%\end{tabular}

%
%\vfill
%
%\newpage
%\restoregeometry




